ReSLLM: Large Language Models are Strong Resource Selectors for Federated Search

Federated search, which involves integrating results from multiple independent search engines, will become increasingly pivotal in the context of Retrieval-Augmented Generation pipelines empowering LLM-based applications such as chatbots. These systems often distribute queries among various search engines, ranging from specialized (e.g., PubMed) to general (e.g., Google), based on the nature of user utterances. A critical aspect of federated search is resource selection - the selection of appropriate resources prior to issuing the query to ensure high-quality and rapid responses, and contain costs associated with calling the external search engines. However, current SOTA resource selection methodologies primarily rely on feature-based learning approaches. These methods often involve the labour intensive and expensive creation of training labels for each resource. In contrast, LLMs have exhibited strong effectiveness as zero-shot methods across NLP and IR tasks. We hypothesise that in the context of federated search LLMs can assess the relevance of resources without the need for extensive predefined labels or features. In this paper, we propose ReSLLM. Our ReSLLM method exploits LLMs to drive the selection of resources in federated search in a zero-shot setting. In addition, we devise an unsupervised fine tuning protocol, the Synthetic Label Augmentation Tuning (SLAT), where the relevance of previously logged queries and snippets from resources is predicted using an off-the-shelf LLM and then in turn used to fine-tune ReSLLM with respect to resource selection. Our empirical evaluation and analysis details the factors influencing the effectiveness of LLMs in this context. The results showcase the merits of ReSLLM for resource selection: not only competitive effectiveness in the zero-shot setting, but also obtaining large when fine-tuned using SLAT-protocol.

==> sections/tables.tex <==










%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|lll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%	fedweb-13 & query & flan-large & name & 0.1144 & 0.1462 & 0.3527 & 0.1052 & 0.1123 \\
%	fedweb-13 & query & flan-large & name-description & 0.1493 & 0.2027 & 0.4463 & 0.0991 & 0.1303 \\
%	fedweb-13 & query & flan-xl & name & 0.1511 & 0.2054 & 0.4123 & 0.1239 & 0.1374 \\
%	fedweb-13 & query & flan-xl & name-description & 0.1766 & 0.2065 & 0.4252 & 0.1603 & 0.1786 \\
%	fedweb-13 & query & flan-xxl & name & 0.2850 & 0.3217 & 0.5647 & \textbf{0.2939} & 0.2747 \\
%	fedweb-13 & query & flan-xxl & name-description & 0.2938 & \textbf{0.3609} & \textbf{0.5786} & 0.2083 & 0.2797 \\
%	fedweb-13 & query & llama2-13b-chat & name & 0.1015 & 0.1339 & 0.3036 & 0.1045 & 0.1069 \\
%	fedweb-13 & query & llama2-13b-chat & name-description & 0.1059 & 0.1379 & 0.3381 & 0.1153 & 0.0999 \\
%	fedweb-13 & query & llama2-7b-chat & name & 0.0683 & 0.0815 & 0.2626 & 0.0273 & 0.0644 \\
%	fedweb-13 & query & llama2-7b-chat & name-description & 0.1054 & 0.1236 & 0.2748 & 0.0889 & 0.1002 \\
%	fedweb-13 & query & mixtral-13b & name & 0.2605 & 0.3059 & 0.5224 & 0.1897 & 0.2492 \\
%	fedweb-13 & query & mixtral-13b & name-description & \textbf{0.2955} & 0.3451 & 0.5319 & 0.2052 & \textbf{0.2915} \\
%	fedweb-13 & query & solar-11b & name & 0.2636 & 0.3029 & 0.5351 & 0.2713 & 0.2486 \\
%	fedweb-13 & query & solar-11b & name-description & 0.2040 & 0.2667 & 0.5085 & 0.1015 & 0.1838 \\ \midrule
%	
%	fedweb-13 & description & flan-large & name & 0.1620 & 0.1862 & 0.4219 & 0.1514 & 0.1411 \\
%	fedweb-13 & description & flan-large & name-description & 0.2136 & 0.2784 & 0.4879 & 0.1865 & 0.1967 \\
%	fedweb-13 & description & flan-xl & name & 0.1789 & 0.2143 & 0.4384 & 0.1939 & 0.1638 \\
%	fedweb-13 & description & flan-xl & name-description & 0.2089 & 0.2454 & 0.4605 & 0.1916 & 0.2037 \\
%	fedweb-13 & description & flan-xxl & name & 0.2984 & 0.3508 & 0.5725 & 0.3392 & 0.2651 \\
%	fedweb-13 & description & flan-xxl & name-description & 0.3060 & 0.3767 & 0.5814 & 0.2218 & 0.2710 \\
%	fedweb-13 & description & llama2-13b-chat & name & 0.1640 & 0.2140 & 0.4129 & 0.1733 & 0.1564 \\
%	fedweb-13 & description & llama2-13b-chat & name-description & 0.1978 & 0.2590 & 0.4363 & 0.1256 & 0.1612 \\
%	fedweb-13 & description & llama2-7b-chat & name & 0.1156 & 0.1467 & 0.3599 & 0.0780 & 0.1045 \\
%	fedweb-13 & description & llama2-7b-chat & name-description & 0.1652 & 0.1973 & 0.3810 & 0.1876 & 0.1607 \\
%	fedweb-13 & description & mixtral-13b & name & 0.2802 & 0.3246 & 0.5562 & 0.2392 & 0.2726 \\
%	fedweb-13 & description & mixtral-13b & name-description & 0.3333 & \textbf{0.3978} & 0.5830 & 0.3109 & 0.3037 \\
%	fedweb-13 & description & solar-11b & name & \textbf{0.3573} & 0.3944 & \textbf{0.5982} & \textbf{0.3809} & \textbf{0.3398} \\
%	fedweb-13 & description & solar-11b & name-description & 0.2917 & 0.3541 & 0.5674 & 0.2692 & 0.2699 \\
%	
%	
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:n}
%\end{table*}
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|llll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&top-n&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%
%fedweb-13 &query & flan-large & example-snippet & 1 & 0.1485 & 0.1918 & 0.4076 & 0.0973 & 0.1527 \\
%fedweb-13 &query & flan-large & example-snippet & 2 & 0.1718 & 0.2106 & 0.4324 & 0.1337 & 0.1545 \\
%fedweb-13 &query & flan-large & example-snippet & 3 & 0.1619 & 0.2079 & 0.4377 & 0.1048 & 0.1464 \\
%fedweb-13 &query & flan-large & example-snippet & 5 & 0.1918 & 0.2367 & 0.4558 & 0.1877 & 0.1701 \\ \midrule
%fedweb-13 &query & flan-xl & example-snippet & 1 & 0.1310 & 0.1605 & 0.3655 & 0.0923 & 0.1280 \\
%fedweb-13 &query & flan-xl & example-snippet & 2 & 0.1369 & 0.1774 & 0.3957 & 0.0844 & 0.1264 \\
%fedweb-13 &query & flan-xl & example-snippet & 3 & 0.1509 & 0.1853 & 0.4131 & 0.1044 & 0.1258 \\
%fedweb-13 &query & flan-xl & example-snippet & 5 & 0.1706 & 0.1982 & 0.4239 & 0.1487 & 0.1498 \\ \midrule
%fedweb-13 & query & flan-xxl & example-snippet & 1 & 0.2179 & 0.2673 & 0.4779 & 0.1404 & 0.2067 \\
%fedweb-13 & query & flan-xxl & example-snippet & 2 & 0.2295 & 0.2884 & 0.5107 & 0.1632 & 0.2156 \\
%fedweb-13 & query & flan-xxl & example-snippet & 3 & 0.2412 & 0.2801 & 0.5126 & 0.1761 & 0.2395 \\
%fedweb-13 & query & flan-xxl & example-snippet & 5 & 0.2382 & 0.2950 & \textbf{0.5155} & 0.1579 & 0.2181 \\ \midrule
%fedweb-13 & query & mixtral-13b & example-snippet & 1 & 0.2375 & 0.2849 & 0.4699 & 0.1633 & \textbf{0.2418} \\
%fedweb-13 & query & mixtral-13b & example-snippet & 2 & \textbf{0.2464} & 0.2861 & 0.4770 & 0.2224 & 0.2102 \\
%fedweb-13 & query & mixtral-13b & example-snippet & 3 & 0.2319 & \textbf{0.2966} & 0.4835 & \textbf{0.2406} & 0.1909 \\
%fedweb-13 & query & mixtral-13b & example-snippet & 5 & 0.2310 & 0.2947 & 0.4993 & 0.1946 & 0.2165 \\ \midrule
%fedweb-13 & query & solar-11b & example-snippet & 1 & 0.2186 & 0.2757 & 0.4850 & 0.1399 & 0.1848 \\
%fedweb-13 & query & solar-11b & example-snippet & 2 & 0.1944 & 0.2479 & 0.4634 & 0.0955 & 0.1784 \\
%fedweb-13 & query & solar-11b & example-snippet & 3 & 0.1883 & 0.2509 & 0.4829 & 0.1914 & 0.1609 \\
%fedweb-13 & query & solar-11b & example-snippet & 5 & 0.1356 & 0.2099 & 0.4595 & 0.1058 & 0.1176 \\ \midrule
%fedweb-13 &description & flan-large & example-snippet & 1 & 0.1457 & 0.1898 & 0.3877 & 0.1323 & 0.1355 \\
%fedweb-13 &description & flan-large & example-snippet & 2 & 0.1871 & 0.2337 & 0.4287 & 0.2331 & 0.1718 \\
%fedweb-13 &description & flan-large & example-snippet & 3 & 0.2024 & 0.2388 & 0.4481 & 0.2068 & 0.1859 \\
%fedweb-13 &description & flan-large & example-snippet & 5 & 0.2070 & 0.2477 & 0.4529 & 0.2540 & 0.1745 \\ \midrule
%fedweb-13 &description & flan-xl & example-snippet & 1 & 0.1701 & 0.2122 & 0.4089 & 0.0997 & 0.1735 \\
%fedweb-13 &description & flan-xl & example-snippet & 2 & 0.1840 & 0.2283 & 0.4442 & 0.1727 & 0.1771 \\
%fedweb-13 &description & flan-xl & example-snippet & 3 & 0.1867 & 0.2236 & 0.4540 & 0.1484 & 0.1788 \\
%fedweb-13 &description & flan-xl & example-snippet & 5 & 0.1788 & 0.2219 & 0.4471 & 0.1302 & 0.1607 \\\midrule
%fedweb-13 & description & flan-xxl & example-snippet & 1 & 0.2795 & 0.3427 & 0.5388 & 0.2201 & 0.2470 \\
%fedweb-13 & description & flan-xxl & example-snippet & 2 & 0.3183 & 0.3810 & 0.5791 & 0.2804 & 0.2863 \\
%fedweb-13 & description & flan-xxl & example-snippet & 3 & \textbf{0.3378} & 0.3844 & \textbf{0.5948} & 0.3102 & 0.3163 \\ 
%fedweb-13 & description & flan-xxl & example-snippet & 5 & 0.3167 & 0.3883 & 0.5835 & 0.2671 & 0.2885 \\ \midrule
%fedweb-13 & description & mixtral-13b & example-snippet & 1 & 0.3024 & 0.3476 & 0.4864 & 0.2840 & 0.2973 \\
%fedweb-13 & description & mixtral-13b & example-snippet & 2 & 0.2824 & 0.3121 & 0.4665 & 0.2547 & 0.2989 \\
%fedweb-13 & description & mixtral-13b & example-snippet & 3 & 0.3234 & 0.3535 & 0.4995 & \textbf{0.3593} & 0.2929 \\
%fedweb-13 & description & mixtral-13b & example-snippet & 5 & 0.3363 & 0.3825 & 0.5279 & 0.3575 & 0.3076 \\ \midrule
%fedweb-13 & description & solar-11b & example-snippet & 1 & 0.3346 & \textbf{0.3905} & 0.5634 & 0.3362 & \textbf{0.3267} \\
%fedweb-13 & description & solar-11b & example-snippet & 2 & 0.3221 & 0.3594 & 0.5411 & 0.3532 & 0.3104 \\
%fedweb-13 & description & solar-11b & example-snippet & 3 & 0.3106 & 0.3522 & 0.5544 & 0.2724 & 0.3068 \\
%fedweb-13 & description & solar-11b & example-snippet & 5 & 0.2417 & 0.3135 & 0.5325 & 0.2091 & 0.2160 \\
%		
%		
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:3}
%\end{table*}
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|lll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%fedweb-14 & query & flan-large & name & 0.1249 & 0.1544 & 0.3450 & 0.0933 & 0.1111 \\
%fedweb-14 & query & flan-large & name-description & 0.2073 & 0.2461 & 0.4818 & 0.1210 & 0.1952 \\
%fedweb-14 & query & flan-xl & name & 0.1484 & 0.1845 & 0.3799 & 0.1097 & 0.1377 \\
%fedweb-14 & query & flan-xl & name-description & 0.1480 & 0.1833 & 0.3882 & 0.1097 & 0.1368 \\
%fedweb-14 & query & flan-xxl & name & 0.2568 & 0.2984 & 0.5428 & 0.2508 & 0.2307 \\
%fedweb-14 & query & flan-xxl & name-description & 0.3231 & 0.3882 & 0.5856 & 0.2087 & 0.3071 \\
%fedweb-14 & query & llama2-13b-chat & name & 0.0977 & 0.1184 & 0.3370 & 0.1047 & 0.0856 \\
%fedweb-14 & query & llama2-13b-chat & name-description & 0.0951 & 0.1226 & 0.3373 & 0.0706 & 0.0988 \\
%fedweb-14 & query & llama2-7b-chat & name & 0.0529 & 0.0717 & 0.2500 & 0.0232 & 0.0441 \\
%fedweb-14 & query & llama2-7b-chat & name-description & 0.0698 & 0.0934 & 0.2435 & 0.0510 & 0.0688 \\
%fedweb-14 & query & mixtral-13b & name & 0.2870 & 0.3431 & 0.5614 & 0.2896 & 0.2572 \\
%fedweb-14 & query & mixtral-13b & name-description & 0.3025 & 0.3555 & 0.5537 & 0.2267 & 0.2642 \\
%fedweb-14 & query & solar-11b & name & \textbf{0.4093} & \textbf{0.4227} & \textbf{0.6115} & \textbf{0.3931} & \textbf{0.3926} \\
%fedweb-14 & query & solar-11b & name-description & 0.2497 & 0.3163 & 0.5406 & 0.0783 & 0.2280 \\ \midrule
%
%fedweb-14 & description & flan-large & name & 0.1810 & 0.1999 & 0.4139 & 0.1924 & 0.1692 \\
%fedweb-14 & description & flan-large & name-description & 0.2581 & 0.2906 & 0.5062 & 0.1881 & 0.2699 \\
%fedweb-14 & description & flan-xl & name & 0.1801 & 0.2092 & 0.4087 & 0.1717 & 0.1866 \\
%fedweb-14 & description & flan-xl & name-description & 0.1996 & 0.2350 & 0.4303 & 0.1609 & 0.2024 \\
%fedweb-14 & description & flan-xxl & name & 0.2705 & 0.3213 & 0.5528 & 0.3408 & 0.2410 \\
%fedweb-14 & description & flan-xxl & name-description & 0.3289 & 0.3898 & 0.5917 & 0.3128 & 0.3022 \\
%fedweb-14 & description & llama2-13b-chat & name & 0.1599 & 0.1945 & 0.4008 & 0.1987 & 0.1401 \\
%fedweb-14 & description & llama2-13b-chat & name-description & 0.1381 & 0.1942 & 0.3965 & 0.0835 & 0.1261 \\
%fedweb-14 & description & llama2-7b-chat & name & 0.0606 & 0.0976 & 0.3132 & 0.0355 & 0.0594 \\
%fedweb-14 & description & llama2-7b-chat & name-description & 0.1067 & 0.1209 & 0.3184 & 0.0874 & 0.1040 \\
%fedweb-14 & description & mixtral-13b & name & 0.2927 & 0.3558 & 0.5680 & 0.2980 & 0.2653 \\
%fedweb-14 & description & mixtral-13b & name-description & 0.3163 & 0.3762 & 0.5797 & 0.2855 & 0.2768 \\
%fedweb-14 & description & solar-11b & name & \textbf{0.4351} & \textbf{0.4509} & \textbf{0.6362} & \textbf{0.3803} & \textbf{0.4363} \\
%fedweb-14 & description & solar-11b & name-description & 0.3205 & 0.3730 & 0.5764 & 0.1999 & 0.2859 \\
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:2}
%\end{table*}
%
%
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|llll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&top-n&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%fedweb-14 & query & flan-xxl & example-snippet & 1 & 0.2431 & 0.2942 & 0.5022 & 0.1293 & 0.2402 \\
%fedweb-14 & query & flan-xxl & example-snippet & 2 & 0.2559 & 0.3058 & 0.5213 & 0.1904 & 0.2372 \\
%fedweb-14 & query & flan-xxl & example-snippet & 3 & 0.2917 & 0.3278 & 0.5412 & 0.2638 & 0.2418 \\
%fedweb-14 & query & flan-xxl & example-snippet & 5 & 0.2621 & 0.3258 & 0.5358 & 0.2128 & 0.2220 \\ \midrule
%fedweb-14 & query & mixtral-13b & example-snippet & 1 & 0.1903 & 0.2426 & 0.4443 & 0.0974 & 0.1771 \\
%fedweb-14 & query & mixtral-13b & example-snippet & 2 & 0.2057 & 0.2665 & 0.4643 & 0.1232 & 0.1906 \\
%fedweb-14 & query & mixtral-13b & example-snippet & 3 & 0.1929 & 0.2508 & 0.4704 & 0.1415 & 0.1675 \\
%fedweb-14 & query & mixtral-13b & example-snippet & 5 & 0.1792 & 0.2582 & 0.4784 & 0.1390 & 0.1526 \\ \midrule
%fedweb-14 & query & solar-11b & example-snippet & 1 & \textbf{0.3095} & \textbf{0.3505} & \textbf{0.5417} & \textbf{0.3061} & \textbf{0.2897} \\
%fedweb-14 & query & solar-11b & example-snippet & 2 & 0.2051 & 0.2581 & 0.4769 & 0.1746 & 0.1680 \\
%fedweb-14 & query & solar-11b & example-snippet & 3 & 0.1739 & 0.2346 & 0.4774 & 0.1204 & 0.1670 \\
%fedweb-14 & query & solar-11b & example-snippet & 5 & 0.1581 & 0.2133 & 0.4617 & 0.1045 & 0.1398 \\ \midrule
%
%fedweb-14 & description & flan-xxl & example-snippet & 1 & 0.3066 & 0.3565 & 0.5468 & \textbf{0.3136} & 0.2777 \\
%fedweb-14 & description & flan-xxl & example-snippet & 2 & \textbf{0.3128} & \textbf{0.3647} & 0.5583 & 0.1998 & 0.2889 \\
%fedweb-14 & description & flan-xxl & example-snippet & 3 & 0.2958 & 0.3594 & \textbf{0.5628} & 0.2511 & 0.2753 \\
%fedweb-14 & description & flan-xxl & example-snippet & 5 & 0.2855 & 0.3472 & 0.5564 & 0.2383 & 0.2645 \\ \midrule
%fedweb-14 & description & mixtral-13b & example-snippet & 1 & 0.2532 & 0.2912 & 0.4652 & 0.1880 & 0.2114 \\
%fedweb-14 & description & mixtral-13b & example-snippet & 2 & 0.2823 & 0.3185 & 0.4774 & 0.2066 & 0.2792 \\
%fedweb-14 & description & mixtral-13b & example-snippet & 3 & 0.2784 & 0.3187 & 0.4879 & 0.1793 & 0.2646 \\
%fedweb-14 & description & mixtral-13b & example-snippet & 5 & 0.2885 & 0.3486 & 0.5168 & 0.2616 & 0.2675 \\ \midrule
%fedweb-14 & description & solar-11b & example-snippet & 1 & 0.2999 & 0.3490 & 0.5413 & 0.3110 & \textbf{0.2917} \\
%fedweb-14 & description & solar-11b & example-snippet & 2 & 0.2465 & 0.3001 & 0.5159 & 0.2335 & 0.2322 \\
%fedweb-14 & description & solar-11b & example-snippet & 3 & 0.2145 & 0.2907 & 0.5118 & 0.1757 & 0.1988 \\
%fedweb-14 & description & solar-11b & example-snippet & 5 & 0.1849 & 0.2628 & 0.4966 & 0.1159 & 0.1549 \\
%		
%		
%		
%		
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:4}
%\end{table*}
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|lll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%		fedweb-13 &/&all-best&/&&0.2990&/&0.1600&0.2100\\
%		fedweb-13 &/&no-info-used&/&&0.1850&/&0.0700&0.1000\\
%		fedweb-13 & query & flan-large & name & 0.7461 & 0.7764 & 0.8515 & 0.6945 & 0.7539 \\
%		fedweb-13 & query & flan-large & name-description & 0.7349 & 0.7789 & 0.8496 & 0.6914 & 0.7499 \\
%		fedweb-13 & query & flan-xl & name & \textbf{0.7557} & \textbf{0.7897} & \textbf{0.8574} & 0.6929 & \textbf{0.7752} \\
%		fedweb-13 & query & flan-xl & name-description & 0.7533 & 0.7830 & 0.8554 & 0.6929 & 0.7676 \\
%		fedweb-13 & query & llama2-7b-chat & name & 0.7302 & 0.7729 & 0.8494 & \textbf{0.7612} & 0.7680 \\
%		fedweb-13 & query & llama2-7b-chat & name-description & 0.7428 & 0.7572 & 0.8397 & 0.6686 & 0.7470 \\ \midrule
%		fedweb-13 & description & flan-large & name & 0.7501 & 0.7932 & 0.8593 & 0.6929 & 0.7714 \\
%		fedweb-13 & description & flan-large & name-description & 0.7459 & 0.7910 & 0.8553 & \textbf{0.7085} & 0.7547 \\
%		fedweb-13 & description & flan-xl & name & \textbf{0.7556} & \textbf{0.7988} & \textbf{0.8622} & 0.6950 & \textbf{0.7857} \\
%		fedweb-13 & description & flan-xl & name-description & 0.7459 & 0.7859 & 0.8540 & 0.6844 & 0.7623 \\
%		fedweb-13 & description & llama2-7b-chat & name & 0.7090 & 0.7613 & 0.8349 & 0.6781 & 0.7562 \\ \midrule \midrule
%		
%		
%		fedweb-14 &/&all-best&/&0.6010&0.7000&/&0.5250&0.5790\\
%		fedweb-14 &/&no-learning-on-human&/&0.4260&0.5170&/&0.2710&0.4040\\
%		fedweb-14 & query & flan-large & name & 0.6265 & 0.6927 & 0.7768 & 0.3060 & 0.6970 \\
%		fedweb-14 & query & flan-large & name-description & 0.6418 & 0.6995 & 0.7809 & 0.3060 & 0.7210 \\
%		fedweb-14 & query & flan-xl & name & 0.6582 & 0.7088 & 0.7855 & 0.3060 & 0.6854 \\
%		fedweb-14 & query & flan-xl & name-description & \textbf{0.6639} & 0.7077 & \textbf{0.7877} & 0.3060 & \textbf{0.7299} \\
%		fedweb-14 & query & llama2-7b-chat & name & 0.5476 & 0.6228 & 0.7111 & \textbf{0.3483} & 0.4816 \\
%		fedweb-14 & query & llama2-7b-chat & name-description & 0.6568 & \textbf{0.7106} & 0.7811 & 0.3060 & 0.6975 \\ \midrule
%		fedweb-14 & description & flan-large & name & 0.6608 & \textbf{0.7158} & 0.7897 & \textbf{0.3230} & \textbf{0.7516} \\
%		fedweb-14 & description & flan-large & name-description & \textbf{0.6736} & 0.7152 & \textbf{0.7902} & 0.3060 & 0.7407 \\
%		fedweb-14 & description & flan-xl & name & 0.6557 & 0.7052 & 0.7833 & 0.3060 & 0.7008 \\
%		fedweb-14 & description & flan-xl & name-description & 0.6608 & 0.6999 & 0.7849 & 0.3060 & 0.7054 \\
%		fedweb-14 & description & llama2-7b-chat & name & 0.6499 & 0.6984 & 0.7683 & 0.3060 & 0.6913 \\
%		fedweb-14 & description & llama2-7b-chat & name-description & 0.6232 & 0.6923 & 0.7577 & 0.3060 & 0.6413 \\
%		
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:2}
%\end{table*}
%


==> table_prompt_labeling.tex <==
%\begin{tabular}{p{2pt}|M{455pt}}
%	\toprule
%	& \textnormal{Prompt} \\
%	\hline
%	\rotatebox[origin=c]{90}{System Prompt} &  Given a query and a web snippet, you must provide a score on an integer scale of 0 to 4 with the following meanings:\linebreak 4 = navigational, this page represents a home page of an entity directly named by the query; the user may be searching for this specific page or site.\linebreak 3 = top relevance, this page or site is dedicated to the topic; authoritative and comprehensive, it is worthy of being a top result in a web search engine.\linebreak  2 = highly relevant, the content of this page provides substantial information on the topic.\linebreak 2 = highly relevant, the content of this page provides substantial information on the topic.\linebreak 1 = minimal relevance, the content of this page provides some information on the topic, which may be minimal; the relevant information must be on that page, not just promising-looking anchor text pointing to a possibly useful page.\linebreak 0 = not relevant, the content of this page does not provide useful information on the topic, but may provide useful information on other topics, including other interpretations of the same query. \\ \midrule
%	
%	\rotatebox[origin=c]{90}{{\centering User Prompt}} & Assume that you are writing a report on the subject of the topic. mark the web snippet according to the previous scale description.\linebreak Query:\linebreak A person has typed \{query\} into a search engine.\linebreak Result:\linebreak Consider the following web snippet:\linebreak —BEGIN WEB Snippet CONTENT—\linebreak \{snippet\}\linebreak —END WEB Snippet CONTENT—\linebreak Instructions:\linebreak Split this problem into steps:\linebreak Consider the underlying intent of the search.\linebreak Measure how well the content matches a likely intent of the query (M)\linebreak Measure how trustworthy the web page is (T).\linebreak Consider the aspects above and the relative importance of each, and decide on a final score (O).\linebreak Produce a JSON of scores without providing any reasoning. Example:\{"M": 2, "T": 1,"O": 1\}\linebreak Results:\\
%	\bottomrule
%\end{tabular}

